MOBIUS: Model-Oblivious Binarized Neural Networks

A privacy-preserving framework in which a computational resource provider receives encrypted data from a client and returns prediction results without decrypting the data, i.e., oblivious neural network or encrypted prediction, has been studied in machine learning that provides prediction services. In this work, we present MOBIUS (Model-Oblivious BInary neUral networkS), a new system that combines Binarized Neural Networks (BNNs) and secure computation based on secret sharing as tools for scalable and fast privacy-preserving machine learning. BNNs improve computational performance by binarizing values in training to $-1$ and $+1$, while secure computation based on secret sharing provides fast and various computations under encrypted forms via modulo operations with a short bit length. However, combining these tools is not trivial because their operations have different algebraic structures and the use of BNNs downgrades prediction accuracy in general. MOBIUS uses improved procedures of BNNs and secure computation that have compatible algebraic structures without downgrading prediction accuracy. We created an implementation of MOBIUS in C++ using the ABY library (NDSS 2015). We then conducted experiments using the MNIST dataset, and the results show that MOBIUS can return a prediction within 0.76 seconds, which is six times faster than SecureML (IEEE S\&P 2017). MOBIUS allows a client to request for encrypted prediction and allows a trainer to obliviously publish an encrypted model to a cloud provided by a computational resource provider, i.e., without revealing the original model itself to the provider.

==> not-used_cryptographic-primitive.tex <==
% -*- coding: utf-8-unix -*-

%メインで使用しているものは秘密分散に基づく秘密計算であるが、OT やGC も実装の一部として利用している。

\if0
\subsubsection{Oblivious Transfer} 

Oblivious transfer (OT) はsender が二つの入力 x0, x1 を受信者に与えたとき、受信者がそのいずれか xbを、anything else あるいは 選んだ xb を明かすことなく、選ぶことができる技術である。
OT は秘密計算の building block としてよく用いられる技術であり、我々が実装に用いたABY framework~\cite{ABY} でも計算の一部として利用されている。
one-round OT はthe protocol in \cite{PVW08} により実装もできるが、これはパワフルな公開鍵暗号を用いている。
symmetric key encryption を一部で用いることで定数ラウンドのまま計算量を削減するOT extension~\cite{IKNP03,ALSZ13} もある。
ABY、すなわち我々の実装で用いた構成は後者である。



\subsubsection{Garbled Circuit}

Yas's Garbled Circuit~\cite{Yao82} は二者間計算においてgarbler とよばれるユーザがboolean function を暗号化し、evaluator であるもう一方がその回路を評価する技術である。
理論上は多者間でも可能であるが、性能上の問題から今日の秘密計算では二者間で用いることが多い。
Garbled Circuit は任意の回路を評価することが可能であることから、秘密計算の機能は非常にrich である。
後述するABY framework~\cite{ABY} においても比較演算など一部の演算を実装するために利用されている。
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{Secret Sharing and Multi-party Computation}
%（秘密分散の話と、それをベースにした秘密計算の概略を書く。）
%\textcolor{red}{Boolean share とArithmetic Share のみ。Yao は現状では問題ありそう。後で場合によって追加。ABY の論文参考に書く}
秘密分散はもともと入力をシェアと呼ばれる形に変換し、あるしきい値以上のシェアがあれば元の情報を復元できる技術である。
秘密計算では、このシェア同士で演算を行うことで、元の入力を隠したまま入力間の計算を行う。
以下ではまず秘密分散の構文を述べ、その後に秘密分散を用いた秘密計算の実現方法について述べる。
最後に本稿で用いる秘密計算の表記について述べる。
%以下ではまず秘密分散の構文を述べ、秘密計算に用いられるShare の種類としてArithmetic Share, Boolean Share, Yao Share を述べる。その後に、それらを包括するフレームワークとして今回実装に用いたABY framework~\cite{ABY} を簡潔にrecallする。

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Syntax}
秘密分散はシェア生成アルゴリズムShare と秘密復元アルゴリズムRecon からなる。
Share は秘密$x$ を入力に取り、任意の$k,n ( k \leq n) \in \mathbb{Z}$ において$n$個のシェア $\{ \jump{ \bm{ x_i} } \}_{i=1}^n$ を作る. 
次にRecon は少なくとも$k$ 個以上のシェアを入力に取り、秘密$x$ を復元する。

\paragraph{秘密計算の実現方法}

秘密計算とは各参加者間で通信を行い，互いに自分の持つ秘密を漏らすことなく統計情報などを計算する手法のことである．
秘密分散を用いた秘密計算では，シェアを持つ参加者間で秘密計算を行うことで，元の秘密情報を復元することなく和や積，論理和，論理積を計算することが出来る．
同様にシェア間の大小比較や等号判定なども可能である。
これらの具体的手法としては文献~\cite{ON07,CH10} などがあり、また、公開ライブラリとしてはABY~\cite{ABY} が知られている。

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\if0
\paragraph{Type of Shares}

\textcolor{red}{以下に述べる各計算はABY フレームワークで用いられているサーバ-クライアントにあるような二者間におけるものであるが、前節で述べた通り我々の提案方式自体では任意の秘密計算を利用可能である。
（SecureML等を見ていると秘密計算の処理は具体的に書いた方が良さそうではあるが、今回はABY は具体的実装の一系統にすぎないため概念のみ書く。なお、GC やOT などは上記の性質程度しかSecureML でもABY でも議論していないため、詳細は省略。）}

Arithmetic Share は主に加法環で定義されるシェアであり、Shamir のSecret Sharing もこの系統に含まれる。
具体的にはシェアを integer modulo で定義することで、入力に関する秘密計算をmodulo 下での加法や乗法など代数計算を通じて利用できる。
\if0  （これ以下はコメントアウト）
秘密$x$ におけるArithmetic Sharing $\jump{ \bm{ x} }^A $としては、first party $P_0$ は乱数$r \in \mathbb{Z}_{2^\ell}$ を生成し、シェアとして$\jump{ \bm{ x} }^A_1 = x-r \bmod 2^\ell$ をsecond party  $P_1$ に送る。
ここで、$P_0$ のシェアは$\jump{ \bm{ x} }_0^A = r \bmod 2^\ell$ となる。
秘密のreconstruction おしては、$x= \jump{ \bm{ x} }^A_0 + \jump{ \bm{ x} }^A_1 \bmod 2^\ell $ を計算する。
なお、以降のすべての計算において、簡単化のため$\bmod 2^\ell $ を省略して記述する。

二つのシェア$\jump{ \bm{ x} }^A$, $\jump{ \bm{ y} }^A$ を与えられたとき、秘密計算における加法と情報は以下の通り計算される。
先ず加法はシェア$\jump{ \bm{ x} }^A_i$ と$\jump{ \bm{ y} }^A_i$ を持つ任意のparty $P_i$ はローカルに$\jump{ \bm{ z} }^A_i = \jump{ \bm{ x} }^A_i + \jump{ \bm{ y} }^A_i$ を計算する。
これを復号すると、$\jump{ \bm{ z} }^A =\jump{ \bm{ x} }^A + \jump{ \bm{ y} }^A$ が秘密計算の結果として得られる。

次に乗法
\fi
次に、Boolean share はXOR で生成されるシェアであり、各値をboolean で表現する。これはブール代数上でのXOR およびAND ゲートを用いることで、Arithmetic Share ではできなかったような論理演算や比較演算を提供できる。
最後にYao Sharing は前節で述べたGarbled Circuit を計算するためのシェアである。GC の各ワイヤにおいて、garbler がそれぞれランダムに設定した鍵を割り当てる。
その後にgarbler は暗号化関数を用いることで二つのinput wire keys におけるそれぞれのゲートのoutput wire keys を暗号化し、evaluator にそのGC およびinput keys を送信する。evaluator はゲートの入力となるinput wire keys を用いてそれぞれのgarbled gate を復号することで、出力wire key を得る。最後にcircuit の暗号文出力をreconstruct する。

ABY framework~\cite{ABY} はこの三つのシェア上での秘密計算を、各シェア間の変換機能と共に提供するC++ 上のフレームワークである。
各シェア毎にできる演算の種類が異なる。具体的にはArithmetic Share は加法および乗法のみが可能である一方、Boolean share およびYao Sharing は加法と乗法に加え、XORと AND の論理演算およびComparison, equality の比較演算が可能である。
また、ABY の内部実装には前述したOT extension を用いている。
We refer the reader to the paper~\cite{ABY} for more details. 
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\paragraph{Notation} 

以下に、本稿で用いる秘密計算の表記について述べる。ここで、任意の整数$a$において、$\jump{ \bm{ a} }$ は$\bm{a}$のシェアとする。

\begin{itemize}
\item  $\jump{ \bm{ a} }  + \jump{ \bm{ b} }$:  
$\jump{ \bm{ a} }$ と $\jump{ \bm{ b} }$ を入力とし、和 $\jump{ \bm{ a+b} }$ を計算

\item  $\jump{ \bm{ a} } + c$:  $\jump{ \bm{ a} }$ と平文$c$ を入力とし、和 $\jump{ \bm{ a + c} }$ を計算

\item  $\jump{ \bm{ a} } *  \jump{ \bm{ b} }$:  $\jump{ \bm{ a} }$ と $\jump{ \bm{ b} }$ を入力とし、 積$\jump{ \bm{ a * b} }$を計算

\item  $\jump{ \bm{ a} } * c$:  $\jump{ \bm{ a} }$ と平文$c$ を入力とし、積 $\jump{ \bm{ a * c} }$ を計算

\item  $\jump{ \bm{ a < b} } $:  $\jump{ \bm{ a} }$ と $\jump{ \bm{ b} }$ を入力とし、大小を比較. 
$\bm{a} < \bm{b} $ の場合、 $\jump{ \bm{ 1} }$ を返し、 $\bm{a} \geq \bm{b}$ の場合は$\jump{ \bm{ 0} } $ を返す. 

\item  $\jump{ \bm{ 0 \leq  b < \frac{p}{2}  } } $:  $\jump{ \bm{ a} }$ を入力とし、$\bm{a}$ が0 以上$\frac{p}{2}$ 未満か判定. 
$0\leq \bm{a} < \frac{p}{2} $ の場合、 $\jump{ \bm{ 1} }$ を返し、 そうでない場合は$\jump{ \bm{ 0} } $ を返す. 

\item $\jump{ \bm{\wedge_{i=1}^n a_i } }$: シェア $\jump{ \bm{ a_i} }$ ($a_i \in \{ 0, 1\}$) を入力とし、その論理積$ \bm{\wedge_{i=1}^n a_i }$ のシェアを出力. 

%\item Reveal($\jump{ \bm{ a} }$): $\bm{a}$ を復号

%\item MatMult($\jump{ \bm{ a} }, \jump{ \bm{ W} }$): $\bm{a}$ と$\bm{W}$ の二つの行列のシェアを入力とし、行列積$\bm{a} \times \bm{W}$ のシェアを出力.   


\end{itemize}
